Do LLMs Consider Security? An Empirical Study on Responses to Programming Questions

The widespread adoption of conversational LLMs for software development has raised new security concerns regarding the safety of LLM-generated content. Our motivational study outlines ChatGPT's potential in volunteering context-specific information to the developers, promoting safe coding practices. Motivated by this finding, we conduct a study to evaluate the degree of security awareness exhibited by three prominent LLMs: Claude 3, GPT-4, and Llama 3. We prompt these LLMs with Stack Overflow questions that contain vulnerable code to evaluate whether they merely provide answers to the questions or if they also warn users about the insecure code, thereby demonstrating a degree of security awareness. Further, we assess whether LLM responses provide information about the causes, exploits, and the potential fixes of the vulnerability, to help raise users' awareness. Our findings show that all three models struggle to accurately detect and warn users about vulnerabilities, achieving a detection rate of only 12.6% to 40% across our datasets. We also observe that the LLMs tend to identify certain types of vulnerabilities related to sensitive information exposure and improper input neutralization much more frequently than other types, such as those involving external control of file names or paths. Furthermore, when LLMs do issue security warnings, they often provide more information on the causes, exploits, and fixes of vulnerabilities compared to Stack Overflow responses. Finally, we provide an in-depth discussion on the implications of our findings and present a CLI-based prompting tool that can be used to generate significantly more secure LLM responses.

==> 06_implications.tex <==
\section{Implications}

%In this section, we explore the implications of our findings from RQ1 and RQ2, grouped into three categories:
Our findings demonstrate critical considerations for leveraging LLMs in SE context. Our study reveals both the potential and limitations of current LLMs in addressing vulnerabilities and informing developers about them. In this section, we discuss actionable insights for developers and model designers aiming to enhance the security awareness of LLMs. These insights not only highlight immediate steps practitioners can take but also point to broader directions for future research and development. We group these implications into three key areas, each addressing a specific stakeholder group: software engineers using LLMs (Section \ref{implications_address_security}), LLM-based tool integrators (Section \ref{implications_tool_integration}), and LLM designers (Section \ref{implications_llm_designers}). Additionally, in Sections \ref{implications_address_security} and \ref{implications_tool_integration} we analyze a total of 100 LLM prompts and responses, experimenting with possible methods of improving security awareness in LLMs' output. Further, we demonstrate a CLI-based tool that serves as a prototype to help achieve these security enhanced responses.

\subsection{Implications for Software Engineers}
\label{implications_address_security}
% Manual Prompt Eng
Our study highlights the critical need for developers to be vigilant about the security of the programming solutions suggested by LLMs. Notably, in RQ1 we found that LLMs rarely issue security warnings autonomously, identifying vulnerabilities in fewer than 40\% of cases under the more favorable experimental settings. This limited detection rate highlights a critical risk: engineers relying solely on LLMs may overlook key security flaws, leaving code vulnerable to exploitation.

One way to make LLM responses more secure could be by providing specific instructions in the prompt \citep{jensen2024software}. 
%One approach to enhancing the security of LLM responses could be for practitioners to deliberately refine their prompts to include specific instructions. %Given certain prompts, LLMs can be more likely to not only address the security vulnerabilities in the prompt but also generate more secure responses. However, 
However, several studies show that developers struggle to create effective LLM prompts ~\citep{chopra2023conversationalchallengesaipowereddata, Nam2024}. Therefore, we experimented with brief prompt additions that would be straight-forward for developers to implement.

% Case Study - Data Sampling
%To explore whether developers can obtain more secure responses from LLMs by modifying their prompts, we experimented with various possibilities in manual prompting. 
We sampled 50 questions from our datasets where none of the LLMs issued any security warnings. To ensure representativeness, we selected 25 instances from the Mentions-Dataset and 25 instances from the Transformed-Dataset. Further, these questions were sampled proportionately to the distribution of vulnerabilities within the corresponding subsets of questions. Next, these prompts were fed to \gpt, the best performing model in our experiments.

We experimented with multiple prompt structures, such as appending the phrase \textit{``Be mindful of potential security implications."} or \textit{``Make the code secure."}, aiming to find a structure that not only maximized the likelihood of LLMs addressing security vulnerabilities but was also concise enough for practical use by developers. We found that the best performing technique included appending the phrase \textit{``Address security vulnerabilities"} to the end of each question. Consequently, we used all modified questions as prompts for three LLMs, resulting in 50 responses. Next, we analyzed the LLM responses to these questions with respect to the RQ1 and RQ2 metrics. The analysis of these 50 responses was performed by two of the authors and followed the same methodology used in answering RQ1 and RQ2 in the main study.

% Editing numbers
Out of the 25 questions from the Mentions-Dataset, \gpt was able to provide security warnings for 19 questions. For the Transformed-Dataset, there was a much less notable enhancement in performance; \gpt issued security warnings for 6 out of the 25 questions. Despite these improvements, \gpt still struggled to identify and warn users about the existence of more than 76\% of the vulnerabilities in the Transformed-Dataset. This indicates that while prompt engineering enhances security awareness, significant limitations remain in LLMs' ability to warn users about vulnerabilities. A significant factor is the challenge LLMs face in accurately detecting vulnerabilities in the first place. Research indicates that even the most advanced  techniques can only achieve an accuracy of 67.7\% \citep{zhou2024large, zhou2024out}.

% Results - RQ2
It is worth noting that when vulnerabilities were pointed out, the LLM always included information about the \textit{causes} and \textit{fixes} in its responses. Exploitations, however, were pointed out in 13/25 instances. In one of the instances, when a user sought help for a Python issue involving an API request and the Flask framework, \gpt addressed the functional problem but also pointed out a security concern, cautioning the user to validate and sanitize all inputs to avoid potential vulnerabilities. Specifically, the model pointed out that directly using user-provided URLs in HTTP requests without proper validation could lead to a Server-Side Request Forgery (SSRF) attack. As such, \gpt identified the cause of the issue (unsanitized user input), recommended input validation as a fix, and noted the potential exploitation through SSRF.% For instance, \llama provided information about the causes, exploits, and fixes for 8/8, 6/8, and 8/8 of the vulnerabilities in the questions of Mentions-Dataset. Similarly, \gpt detailed the causes, exploits, and fixes of all four instances where it pointed out vulnerabilities in the Transformed-Dataset. %These examples suggest that despite the limitations of LLMs in pointing out vulnerabilities, once identified, the LLMs are effective at conveying sufficient security-related information.

% Takeaway
The overall performance of \gpt using the ``security-aware'' prompts highlights the potential influence of prompts on the security of the LLM responses. Although practitioners can rely on such simple prompt engineering techniques to implement more secure programming solutions, they should exercise caution as this method, in some instances, does not result in more secure LLM responses.

% Limitations
% Our findings reveal significant gaps in the security awareness of LLMs, indicating a need for improvements in their design and training. While we found that LLMs can be powerful tools in describing the causes, exploits, and fixes of vulnerabilities, this effectiveness is contingent upon the LLMs' ability to identify vulnerabilities and warn the user in the first place (40\% in the best case). The performance gets worse when LLMs encounter unseen data or new programming problems (as low as 12.6\%). Moreover, we found that certain vulnerabilities, such as CWE-312 and CWE-798, are more likely to be identified by LLMs compared to other CWEs.

% Nonetheless, we can still foster better performance in various tasks by strategically manipulating prompts, thus optimizing the immediate utility of current LLM capabilities. In particular, grounding the prompts, by adding additional contextual or analytical information, makes them more specific and meaningful for the LLM \cite{}.



% CodeQL
\subsection{Implications for Tool Integration in Software Development}
\label{implications_tool_integration}
% \Experiments with the CodeQL?

% LLM Designs


% Integrating Static Analysis Tools into Prompts
% To address this effectively and immediately, we propose an experimental approach that integrates static analysis tools, such as CodeQL, into the prompt generation process for LLMs. By automatically running these tools on the code snippets provided in prompts and including the vulnerability analysis in the input, we can significantly enrich the context for the LLM. This method serves as an extension of the Retrieval Augmented Generation (RAG) technique, leveraging existing security data to enhance the model’s output. This not only improves the relevance and security-awareness of the responses but also aligns with ongoing efforts to augment LLM capabilities through enriched contextual data.
%However, to effectively and immediately 
To address the limitations of LLMs in identifying and mitigating vulnerabilities, alternative approaches have been proposed. 
%For instance, Pearce et al. have demonstrated the integration of outputs from static analysis tools, such as CodeQL and C sanitizers, into LLM prompts \cite{pearce2023examining}. This approach was implemented as a zero-shot strategy, where LLMs were tasked with fixing vulnerabilities. 
For instance, Pearce et al. demonstrated integrating outputs from static analysis tools, such as CodeQL and C sanitizers, into LLM prompts as a zero-shot strategy for fixing vulnerabilities \cite{pearce2023examining}. 
Building on the same idea, we explored using this technique to examine how well LLMs provide relevant security warnings and information when responding to general programming questions.


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{side_by_side_example.pdf}
    \caption{\textcolor{blue}{Comparison of the LLM’s original functionality-focused response (left) and its subsequent security-focused response (right). On the right, we observe that explicit mention of vulnerability caused the model to overlook the main question.}}
    \label{fig:side_by_side_example}
    % \vspace{-1em}
\end{figure*}

% "Address Vulnerability: Des
We use the same 50 questions used in Section \ref{implications_address_security} to experiment with this approach. Having analyzed each question's extracted code snippets with CodeQL, we add CodeQL's description of the detected vulnerabilities to the end of each question, using the phrase \textit{``Address security vulnerability: \textless Vulnerability Description \#1\textgreater{} Address security vulnerability: \textless Vulnerability Description \#2\textgreater{}..."}. After prompting the \gpt with these prompts, the LLM responses were again analyzed with respect to RQ1 and RQ2. Here, similar to the previous section, the authors manually carried out the analysis.

% Results
Upon providing \gpt with the output of CodeQL, it was able to identify and address vulnerabilities in 24/25 questions from the Mentions-Dataset. Further, the \gpt was able to identify and address 20/25 vulnerabilities for the Transformed-Dataset. However, for six questions, the LLMs ignored the CodeQL output and proceeded to answer the main question without necessarily fixing the code. Consistent with our previous results, the model provided information about the causes, exploits, and the fixes of almost all the vulnerabilities it pointed out. Overall, this technique significantly performed better than the manual prompt engineering technique (Section \ref{implications_address_security}).


% \textcolor{blue}{We also examined whether emphasizing security affected the overall functional correctness of the LLM's answers. In 45 out of the 50 augmented responses, \gpt still adequately addressed the user's original query while highlighting or fixing security vulnerabilities. However, in 4 instances, the LLM primarily focused on resolving the discovered vulnerabilities, neglecting the user’s main question.Figure \ref{fig:side_by_side_example} illustrates one of these scenarios. In this example, the user asks about a data-processing task and includes a snippet that inserts user-provided text into the DOM, i.e., an XSS risk. Without any security-specific instruction, the LLM simply solves the data-processing problem while ignoring the XSS. However, after we add the instruction “Address security vulnerability: DOM text reinterpreted as HTML,” the LLM emphasizes sanitizing user input and preventing XSS while neglecting the user’s original question. This behavior illustrates a potential trade-off between functionality and security, highlighting the challenge of balancing the two objectives in real-world usage.}
\textcolor{blue}{We also examined whether modifying the prompts affected the overall functional correctness of the LLM's answers. In 46 out of the 50 responses, \gpt adequately addressed the user’s primary concern while fixing and/or acknowledging the security vulnerabilities. However, in 4 instances, the LLM’s response only addressed the security issue and completely overlooked the user’s main query. Figure \ref{fig:side_by_side_example} illustrates one such scenario where the question seeks guidance on preventing multiple database entries for the same user. Note that the user's code insecurely handles logging credentials, introducing a potential security risk. Without a security-specific prompt, the LLM addresses the core issue, ignoring the vulnerability (Figure \ref{fig:side_by_side_example} - left panel). After integrating the CodeQL findings into the prompt, the LLM only addresses the logging and credential handling vulnerabilities while neglecting the main question (Figure \ref{fig:side_by_side_example} - right panel). This example demonstrates how emphasizing security can sometimes overshadow the original problem and highlights the challenge of balancing these objectives in real-world usage.}

%The comparable performance between this approach and the manual prompt engineering (Section \ref{implications_address_security}) indicates the possibility of an automatic process that enables more security-aware LLM responses. 
\textcolor{blue}{Despite the challenges, several opportunities exist for integrating LLMs with SE tools in the development workflows.} For instance, static analysis tool like CodeQL can be used to preprocess code snippets to outline specific security vulnerabilities in the prompt. The identified vulnerability can then be added as meta data to the prompt, providing the LLM with clearer directions on what issues need addressing. Such integration could enhance the LLM's ability to generate secure code and streamline vulnerability detection and mitigation.  

To further demonstrate the potential of this approach in practice, we developed a prototype CLI-based tool that automates the integration of static analysis feedback into LLM prompts. The tool automatically extracts the Python or JavaScript code from developer queries, analyzes the code snippets using CodeQL, and integrates the detected vulnerabilities into the LLM’s prompts using the above-mentioned prompt structure. Figure \ref{fig:prototype_screenshot} shows an example interaction using our prototype, highlighting the security enhanced response from the \gpt. In this example, the developer's prompt does not mention any security risks. When prompted directly with this question, \gpt does not address this issue in the user's code. However, after integrating the CodeQL feedback, the LLM not only identified the risk of log injection but also warned the user about its potential exploits and suggested fixes, such as sanitizing user input using the \textit{sanitize} function from the \textit{validator} library. This example demonstrates how integrating static analysis tools into LLM pipelines can effectively enhance security awareness in LLM responses and increase the proactive mentions of insecure vulnerabilities in developers' code.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{fig_pipeline_white.pdf}
    \caption{Left: The original user prompt featuring vulnerable code. Right: The LLM's response after prompt modification (integrating CodeQL feedback). Both the prompt and response have been abbreviated for presentation clarity.}
    \label{fig:prototype_screenshot}
    % \vspace{-1em}
\end{figure*}


% \subsection{Implications for LLM Designs}
%\subsection{Implications for Automated Prompt Engineering}
%\subsection{Using LLMs for Programming Assistance}
\subsection{Implications for LLM Designers}
\label{implications_llm_designers}

Overall, our findings highlight substantial gaps in the security awareness of LLMs, emphasizing the need for design and training improvements. Based on the results of RQ1, the best performance we observed in issuing security warnings was only 40\%, which declines even further in the Transformed-dataset, dropping to as low as 12.6\%. This significant disparity in performance across datasets suggests that LLMs require substantial modifications to improve the attention to security in their responses. Addressing these gaps might involve acquiring additional high-quality training data, or domain-specific fine-tuning for SE. %, or even new model architectures. %, such enhancements are outside the scope of this discussion. 

Moreover, our study suggests that LLMs' lack of attention to security extends beyond code generation to the natural language they produce in software engineering-related discussions. This broader issue indicates the need to evaluate the security of LLM-generated content, particularly in the explanations, advice, and recommendations provided to developers. Future research could establish standardized methods for assessing LLM security awareness within software engineering contexts, focusing not only on the code produced but also on the security of LLM-provided guidance. This dual approach to security—encompassing both code and conversational context—could enable more robust, security-conscious LLM designs that better serve practitioners in high-stakes environments.

==> 07_threats_to_validity.tex <==
\section{Threats to Validity}


\textbf{Internal Validity:} An LLM may appear to address the security flaws within a given prompt; however, if the prompt was a part of the LLM's training data, the generated response could merely reflect that information, and not the model's generalizability. To counteract this threat, we created the Transformed-Dataset. This dataset includes transformed SO questions devoid of any security mentions, either in questions or responses. Therefore, we expect 
%that none of the three LLMs has encountered these specific questions or any notions of security regarding them, allowing us to assess the model's capability to identify and address security issues in new data.
none of the three LLMs to have encountered these specific questions or related security concepts, allowing us to assess their ability to address security issues in new data. 

\textbf{External Validity:} The results of our study may not generalize to all LLMs or programming questions. %\textcolor{blue}{For instance, the inclusion of other LLMs, such as code-specific models that place a heavier emphasis on code and provide more concise natural language output, is outside the scope of our study and can be explored further in future work.} However, to investigate the security awareness of cutting-edge LLMs, we included three of the most popular models: \gpt, \llama, and \claude. Further, we collected our datasets from a SO dump spanning 9 years (March 2015-March 2024). We selected questions related to two popular programming languages, Python and JavaScript, to ensure  our findings adaptable to a wide range of development scenarios and questions.
\textcolor{blue}{One key limitation of our study is the exclusion of code-specific LLMs, such as DeepSeek-Coder \cite{deepseekcoder} and Qwen-Coder \cite{hui2024qwen2}, which are designed specifically for code-related tasks. These models place a stronger emphasis on code comprehension and may yield different security-related responses compared to the conversational LLMs we evaluated. While our focus was on conversational LLMs widely used in developer interactions, we acknowledge that analyzing the security awareness of code-specific models is an important avenue for future research. In investigating the security awareness of conversational LLMs, however, we included three of the most popular models: \gpt, \llama, and \claude. Further, we collected our datasets from a SO dump spanning 9 years (March 2015–March 2024). We selected questions related to two popular programming languages, Python and JavaScript, to ensure our findings remain adaptable to a wide range of development scenarios and questions.}


\textbf{Construct Validity:} Much of the qualitative analysis done throughout this work has been the result of manual efforts by the authors. To ensure the reliability of our analyses, we %used Cohen's Kappa to measure inter-rater agreement among the authors. 
calculated the inter-rater agreement using Cohen Kappa coefficient, and iteratively discussed and resolved conflicts to reach sufficient agreement ($>$ 0.6). 
We chose to use an static analysis tool for automatically identifying the security vulnerabilities in code snippets which can sometimes produce false positives or false negatives. To mitigate this threat, in line with prior work, we relied on CodeQL, as it offers higher precision at the expense of a lower recall. As a result, by prioritizing precision, we ensure that the vulnerabilities included in our dataset are more accurate and reliable.

% although commonly used, codeql performs best in real-world projects and codebases and not necessarily code snippets from questions. The differences in the code of the development and the deployment environment affects the performance of CodeQL % Hard coded credentials example

% There can be instances of the LLM providing improved code (security-wise) to the vulnerable code they have been prompted with. In these instances the LLM may not provide any mention of the existing vulnerability in the prompt. (we could start running codeql on the code snippets of the LLMs to see if the vulnerability still exists or not)

% Could the vulnerabilities that were also pointed out by SO users, easier to detect?


==> 08_related_work.tex <==
\section{Related Work}

% \subsection{Large Language Models in Software Engineering}
% The impact of LLMs on SE practices
% Large language models have deeply influenced various aspects of software engineering, offering new possibilities for code generation, summarization, and debugging by answering queries related to software development practices. Tools like GitHub Copilot \cite{githubcopilot}, OpenAI's GPT series \cite{openai2023chatgpt}, Anthropic's Claude \cite{claude}, and Meta's LLaMA\cite{llama} generate code snippets based on natural language prompts, accelerating the development process and reducing the time spent on repetitive coding tasks. Developers regularly use LLMs for code generation, debugging, and general information retrieval purposes \cite{saud2024chatting}. 

% General study of LLMs in SE
% Given the significant influence of LLMs on software engineering practices, researchers have extensively studied the impact of LLMs in the field. A study by Das et al. analyzed the interactions of developers with ChatGPT, revealing its utility in tasks such as code generation, comprehension, debugging, ideation, and validation \cite{das2024investigating}. Their findings also indicate that developers frequently leverage ChatGPT during the ideation phase, receiving suggestions, new approaches, and potential solutions to their problems in form of \textit{natural language}. Likewise, developers use LLMs to summarize complex code segments, making it easier to understand and modify existing codebases.

Researchers have studied the adoption of LLMs in security-related software engineering tasks. Multiple studies have explored the possibilities and limitations of LLMs in vulnerability detection \citep{zhou2024large, noever2023can, bakhshandeh2023using, purba2023software, cheshkov2023evaluation, wang2023defecthunter, liu2023harnessing}. Some of these studies have demonstrated the superior performance of LLMs compared to traditional methods such as static analysis tools \citep{zhou2024large, noever2023can, bakhshandeh2023using}, while others have highlighted the shortcomings of LLMs, particularly their tendency to generate false positives \citep{purba2023software, cheshkov2023evaluation, Banerjee23}. Additionally, LLMs have been employed to detect malicious code \citep{plate, eli}, generate test cases \citep{yao2023llm, zhang2023well}, and to fix defective and/or vulnerable code \citep{jiang2023impact, pearce2023examining, xia2022practical, jin2023inferfix}. Beyond the use of LLMs in performing security-related tasks, researchers have also studied the security issues caused due to the use of LLMs. We discuss some of these studies in Sections \ref{concerns_with_llms_in_se} and \ref{concerns_in_llms_vs_SO}.

\subsection{Security Concerns with using LLMs} 
\label{concerns_with_llms_in_se}
% Code generation LLMs
% Following the widespread adoption of LLMs by developers, many researchers have shown interest in studying how this integration impacts the security of the produced software. 
Numerous studies studied the security of the code generated by LLMs. %In one of the earlier works in this area, 
\cite{pearce2022asleep} examined security of the code generated by GitHub's Copilot \citep{githubcopilot}. They found that around 40\% of the code generated by Copilot contained vulnerabilities when analyzed with CodeQL \citep{GitHubCodeQL}. Other studies have also evaluated the security of code from different code generation models, comparing it to human-written code \citep{siddiq2022securityeval, asare2023github}. %In their study, Copilot was prompted to generate code that, if not implemented properly, would introduce vulnerabilities to software. The generated code was then analyzed using CodeQL \cite{GitHubCodeQL}, revealing that approximately 40\% of the Copilot's code contained vulnerabilities. Other studies have examined the security of the code written by different code generation models and even compared it to human-written code \cite{siddiq2022securityeval, asare2023github}. %Similar studies have also taken into account conversational LLMs, evaluating the security of code generated by models such as ChatGPT \cite{khoury2023secure, siddiq2024quality}. Unlike these studies, our work highlights the security of the LLM-generated responses in form of natural language.
% In a different study, Siddiq et al published an evaluation dataset for assessing the security of the LLM generated code snippets \cite{siddiq2022securityeval}. In addition, they use this dataset to find the security vulnerabilities in code generated by Copilot and Incoder \cite{fried2022incoder}. In a more recent publication, researchers compared the security of the Copilot generated code with that of human developers, concluding that Copilot is less likely to generate vulnerable code \cite{asare2023github}.

% Conversational LLMs
In addition to the code generation models such as Insider and Copilot, LLMs have also been scrutinized for the security of their generated code. \cite{khoury2023secure} tasked ChatGPT with generating 21 programs likely to contain vulnerabilities. The results revealed that ChatGPT only provided secure code in five out of 21 programs. %and was able to fix its generated code in seven other cases \cite{khoury2023secure}.
Similarly, \cite{siddiq2024quality} used CodeQL, Bandit, and Pylint to evaluate the security of code generated by ChatGPT, finding a number of security issues related to improper resources and exception management.

LLMs have been proven useful in detecting security vulnerabilities~\cite{lu2024grace, zhou2024large, thapa2022transformer, yao2024survey}. Based on these studies, and supported by the preliminary validation of our motivational study we initially hypothesized that LLMs possess the security knowledge needed to warn users of potential threats. However, our findings show that LLMs do not always recognize when or how to apply this knowledge effectively. Different from previous studies, our work focuses on determining LLMs' abilities in proactive prevention i.e., proactively identifying and flagging vulnerabilities. To the best of our knowledge, we are the first to assess LLMs'  capability in communicating critical information (causes, exploits, and fixes) to enhance developer understanding and  encourage the adoption of secure coding practices. %Our evaluation examines the ability of LLMs for \textbf{proactive prevention} i.e., proactively identifying and flagging vulnerabilities. While we might not yet expect this from LLMs, this will become critical as AI-driven tools become more integrated into development workflows. 
%\textcolor{blue}{add a short sentence how our work is different from rest and what are we contributing}%Unlike these studies, our work does not focus on the code, but rather natural language output of LLMs. By analyzing how LLMs use natural language to communicate, or fail to communicate, vital security information, we aim to understand their role in shaping developers' security awareness.% and practices.

% Prompt engineering & Output optimization
% The concerns regarding the LLM approaches in many software engineering tasks have inspired researchers to seek methods for improving the LLM outputs. Prompt engineering \cite{homoliak2024enhancing, pearce2022asleep, yetistiren2022assessing} and output optimizing \cite{vernikos2023small, wang2023factcheck} are among the techniques, commonly used to improve LLM generated content. One notable study demonstrated the use of scenario-specific, iterative, and general clause methods to rephrase the prompts of GitHub Copilot in order to enhance the security of the generated code \cite{homoliak2024enhancing}. The use of certain prompt engineering techniques in our work is meant to improve the performance of the LLMs with respect to our own particular metrics, as further described in Section \ref{methodology_case_study}.

% Offensive LLM applications
% It's worth noting that the concerns about the use of LLMs in the software space extend beyond the limitations of LLMs in performing certain software engineering tasks. As pointed out by Yao et al., LLMs can and have been actively used for offensive applications\includecomment{, against security and privacy}\cite{yao2024survey}. These offensive applications can range from hardware to user-level attacks. In an example of an OS-level attack, Happe and Cito demonstrated how providing ChatGPT with an SSH connection to a Linux virtual machine in a closed feedback loop resulted in a successful privilege escalation attack \cite{happe2023getting}. The offensive applications of LLMs are, however, beyond the scope of this study.


\subsection{Stack Overflow vs. LLMs: Security Implications} 
\label{concerns_in_llms_vs_SO}
% Intro
Popularity of Stack Overflow has been significantly impacted by the emergence of LLMs\citep{da2024chatgpt}. Despite the varying quality of LLM-generated answers, many developers prefer ChatGPT due to their well-articulated language \citep{kabir2024stack}. While a rich body of literature on SO and the security concerns associated with its usage remains \citep{yang2016security, licorish2021contextual, fischer2017stack, zhang2018code}, researchers are still exploring the consequences of relying on LLM responses instead of user-provided SO responses. 
% This transition has inspired a number of studies to compare user-generated responses on SO to LLM-generated responses. 
% often comparing LLM-generated code to traditional user-generated content on SO. 

% Security-focused comparison of SO & LLMs
\cite{da2024chatgpt} compared the reliability of LLM-generated responses to user-provided answers on SO. Their results indicate that despite a high degree of textual similarity, the LLM responses are not reliable. Furthermore, they report a considerable decline in user activity on SO since the introduction of ChatGPT. %,  suggesting that some developers are relying on LLM responses to answer their questions instead of SO.
% They They also compared the reliab responses to the answers generated by LLaMA-2 and ChatGPT-3.5 \cite{da2024chatgpt}. Their results indicate a high degree of textual similarity between ChatGPT and SO responses. %with the unpopular features of frameworks and libraries to be the most challenging questions for the LLMs. 
In another study, ChatGPT was prompted with 517 SO questions, revealing that 52\% of the responses contained incorrect and fabricated information\citep{kabir2024stack}. %Regardless, 35\% of the involved study participants still preferred the LLM responses to the SO responses, overlooking the incorrect information \cite{kabir2024stack}. 
% Others have shown 74\% of the user-provided responses and 71\% of the ChatGPT-generated responses to the same privacy-related SO questions to be accurate \cite{delile2023evaluating}. and discovered multiple vulnerabilities in ChatGPT's code, responding to SO security questions \cite{hamer2024just}.
\cite{delile2023evaluating} have shown that 74\% of the user-provided responses and 71\% of the ChatGPT-generated responses to privacy-related SO questions are accurate. In another study, \cite{hamer2024just} discovered multiple vulnerabilities in ChatGPT's code when responding to SO security questions. While they focused on whether LLMs generate vulnerable code, we aim to assess if LLMs, when prompted with vulnerable code, inform users about the security implications.
%In contrast to these studies, our work does not attempt to assess the correctness of the LLM-generated responses to SO questions. Instead, we aim to understand whether LLMs, prompted with vulnerable code, would inform users about the security implications of their code.

% In another study, researchers, prompted ChatGPT with 92 privacy related SO questions and manually analyzed both the responses Finding 74\% of the SO responses and 71\% of the ChatGPT responses to be accurate \cite{delile2023evaluating}. Further, Hmaer et al. prompted ChatGPT with security-related SO questions and used CodeQL to detect existing vulnerabilities, finding a number of vulnerabilities both in SO and ChatGPT answers \cite{hamer2024just}.  In contrast to these studies, our work does not attempt to assess the correctness of the LLM-generated responses to SO questions. Instead, we aim to understand whether LLMs, prompted with a question that contains vulnerable code, would inform users about the security implications of their code or if they only answer the question.

% Overall Distinguishing Factors of our Work
Overall, our work is distinct in two ways. First, instead of assessing the security of LLM-generated code, we evaluate the natural language responses. Second, unlike studies that prompt LLMs with specific security-related tasks such as vulnerability detection, we deliberately avoid any mention of security in our prompts. Instead, we present LLMs with only SO questions that contain insecure code. This emulates real-life programming Q\&A and allows us to evaluate the security awareness of LLMs in practical applications. %emulating real-life programming Q\&A. This allows us to evaluate the security-awareness of LLMs and their ability to inform users about the vulnerable code. %in various plausible real-world scenarios.
% We aim to understand whether LLMs proactively contribute to security awareness in software development or if they potentially encourage insecure practices by turning a blind eye to the users' insecure code. 
% Lastly, our use of prompt engineering methods is meant to improve the security awareness of the LLM answers with respect to our particular specific metrics, described in Section \ref{methodology_case_study}, as opposed to common tasks such as vulnerability detection or secure code generation.


==> 09_conclusions.tex <==
\section{Conclusions}
This paper presents the first study to examine the security awareness of three popular LLMs when answering programming-related questions.
%In this work, we offer a first look into the security awareness with which LLMs respond to programming questions. Our motivational study showed that ChatGPT rarely mentions security when answering developers' questions. %and that often these mentions are limited to certain types of vulnerabilities.
In our motivational study, ChatGPT demonstrated potential in offering developers relevant security-related information and context-based solutions for writing secure code. 
%Our motivational study showed ChatGPT’s potential to identify security vulnerabilities and provide context-specific information to developers, promoting safe coding practices.
These findings inspired us to conduct a deeper investigation into the capabilities of other popular LLMs.
We prompted three popular LLMs, \gpt, \llama and \claude, with SO questions containing vulnerable code and evaluated their responses. 

Our results indicated the underwhelming performance of all three LLMs in pointing out the security vulnerabilities. We observed even lower performances when prompting LLMs with questions from Transformed-Dataset which, indicates the limitations of these models in generalizing their learned data. 
Additionally, we observed that LLMs are more likely to point out certain vulnerabilities, specially those related to the improper management and protection of sensitive information (e.g., CWE-532, CWE-321, CWE-798) compared to those involving external control of file names or paths (e.g., CWE-400). 
%such as CWE-532 (Insertion of Sensitive Information in Log File), CWE-321 (Use of Hard-coded Cryptographic Key), and CWE-798 (Use of Hard-Coded Credentials). Is to be noted that, in instances where LLMs identified the vulnerabilities, they provided more comprehensive information than Stack Overflow posts. 
%Evaluating the security warnings offered by the LLMs, we found that all models consistently detailed the causes, potential exploits, and possible fixes of vulnerabilities, to better inform users. 
%This information was often comprehensive and therefore more helpful in raising user's awareness compared to the responses found on SO.
% Lastly, we conducted a case study investigating the performance of all LLMs in detecting vulnerabilities, given slightly modified prompts. By adding the phrase ``Address security vulnerabilities" to the end of each question, LLMs detected 40\% of the vulnerabilities for questions in Transformed-Dataset where no LLM originally issued a security warning.
% Finally, we discussed the security implications of our findings in future tool designs. We also suggest a simple, practical prompt engineering technique that developers can adopt to receive more security-aware LLM responses. 

While some of our findings align with existing research on security flaws in LLM-generated content, our approach addresses a crucial gap by focusing on real-world scenarios where developers seek general coding assistance without explicitly considering security, which is common in interactions. By selecting prompts without explicit security mentions, we simulate typical developer interactions in which security concerns are often overlooked, highlighting a key risk: \textit{LLMs often overlook insecure practices and inadvertently reinforce them}. This insight, when coupled with the prompting techniques we propose, could help developers elicit more security-aware responses from LLMs, thus promoting secure coding practices. 

In general, our findings have the following key implications. For software engineering practitioners, prompt engineering can be a practical tool to promote security-aware LLM outputs, though limitations remain; integrating tools like CodeQL may further aid developers in outlining vulnerabilities. For researchers, the results point to the importance of evaluating both code and natural language guidance from LLMs and highlight opportunities for fine-tuning models to generate more security-aware responses. For LLM designers, there is a need for models that proactively identify security issues, perhaps through enhanced training or fine-tuning with high-quality, domain-specific data. 
\newline\newline
\textbf{Data Availability:} The replication package of our study, including the datasets, code, and analysis instructions are available at: \url{https://figshare.com/s/4f85174699540324fc4d}.
